Heavy ions at the Future Circular Collider

The Future Circular Collider (FCC) Study is aimed at assessing the physics potential and the technical feasibility of a new collider with centre-of-mass energies, in the hadron-hadron collision mode, seven times larger than the nominal LHC energies. Operating such machine with heavy ions is an option that is being considered in the accelerator design studies. It would provide, for example, Pb-Pb and p-Pb collisions at sqrt{s_NN} = 39 and 63 TeV, respectively, per nucleon-nucleon collision, with integrated luminosities above 30 nb^-1 per month for Pb-Pb. This is a report by the working group on heavy-ion physics of the FCC Study. First ideas on the physics opportunities with heavy ions at the FCC are presented, covering the physics of the Quark-Gluon Plasma, of gluon saturation, of photon-induced collisions, as well as connections with other fields of high-energy physics.

==> 01-introduction/report.tex <==
% Few simple rules to ensure that we you can pdfplatex your section
% locally, while maintaining the ability to pdflatex the full
% document from the home directory:

% Don't touch any of the calls in this file. 

% If you want to break the section into multiple subsection files, embed
% the \input{subsectionX} calls into the file section.tex

% Subsection files must then stay in the same folder as section.tex,
% and their figures should all stay in the figs/ subdirectory

% All references should included using the bibtex format, and must be
% added to the master report.bib file sitting in the main directory

% If you want to add new tex macros (mostly definitions or new
% commands), include them in your local section.tex file. But first
% make sure you are not overriding the macros already included in the
% main_macros.tex file sitting in the home directory. When processing
% the whole report, each subsection will then call properly its own
% macros, and properly use the master macros

% If you want to collect your macros in a file, you should then input
% it from the file section.tex or 
% from the subsection files, but it should NOT be called
% ``main_macros.tex'' (e.g. call it sectionname_macros.tex)

\input{../header}
\input{../title}
\input{../main_macros}

\input{section}

\bibliographystyle{../report}
\bibliography{../report}

\end{document}




==> 02-machine/report.tex <==
% Few simple rules to ensure that we you can pdfplatex your section
% locally, while maintaining the ability to pdflatex the full
% document from the home directory:

% Don't touch any of the calls in this file. 

% If you want to break the section into multiple subsection files, embed
% the \input{subsectionX} calls into the file section.tex

% Subsection files must then stay in the same folder as section.tex,
% and their figures should all stay in the figs/ subdirectory

% All references should included using the bibtex format, and must be
% added to the master report.bib file sitting in the main directory

% If you want to add new tex macros (mostly definitions or new
% commands), include them in your local section.tex file. But first
% make sure you are not overriding the macros already included in the
% main_macros.tex file sitting in the home directory. When processing
% the whole report, each subsection will then call properly its own
% macros, and properly use the master macros

% If you want to collect your macros in a file, you should then input
% it from the file section.tex or 
% from the subsection files, but it should NOT be called
% ``main_macros.tex'' (e.g. call it sectionname_macros.tex)

\input{../header}
\input{../title}
\input{../main_macros}

\input{section}

\bibliographystyle{../report}
\bibliography{../report}

\end{document}




==> 03-qgpsoft/report.tex <==
% Few simple rules to ensure that we you can pdfplatex your section
% locally, while maintaining the ability to pdflatex the full
% document from the home directory:

% Don't touch any of the calls in this file. 

% If you want to break the section into multiple subsection files, embed
% the \input{subsectionX} calls into the file section.tex

% Subsection files must then stay in the same folder as section.tex,
% and their figures should all stay in the figs/ subdirectory

% All references should included using the bibtex format, and must be
% added to the master report.bib file sitting in the main directory

% If you want to add new tex macros (mostly definitions or new
% commands), include them in your local section.tex file. But first
% make sure you are not overriding the macros already included in the
% main_macros.tex file sitting in the home directory. When processing
% the whole report, each subsection will then call properly its own
% macros, and properly use the master macros

% If you want to collect your macros in a file, you should then input
% it from the file section.tex or 
% from the subsection files, but it should NOT be called
% ``main_macros.tex'' (e.g. call it sectionname_macros.tex)

\input{../header}
\input{../title}
\input{../main_macros}

\input{section}

\bibliographystyle{../report}
\bibliography{../report}

\end{document}




==> 04-qgphard/report.tex <==
% Few simple rules to ensure that we you can pdfplatex your section
% locally, while maintaining the ability to pdflatex the full
% document from the home directory:

% Don't touch any of the calls in this file. 

% If you want to break the section into multiple subsection files, embed
% the \input{subsectionX} calls into the file section.tex

% Subsection files must then stay in the same folder as section.tex,
% and their figures should all stay in the figs/ subdirectory

% All references should included using the bibtex format, and must be
% added to the master report.bib file sitting in the main directory

% If you want to add new tex macros (mostly definitions or new
% commands), include them in your local section.tex file. But first
% make sure you are not overriding the macros already included in the
% main_macros.tex file sitting in the home directory. When processing
% the whole report, each subsection will then call properly its own
% macros, and properly use the master macros

% If you want to collect your macros in a file, you should then input
% it from the file section.tex or 
% from the subsection files, but it should NOT be called
% ``main_macros.tex'' (e.g. call it sectionname_macros.tex)

\input{../header}
\input{../title}
\input{../main_macros}

\input{section}

\bibliographystyle{../report}
\bibliography{heavyflavour}

\end{document}




==> 05-smallx/report.tex <==
% Few simple rules to ensure that we you can pdfplatex your section
% locally, while maintaining the ability to pdflatex the full
% document from the home directory:

% Don't touch any of the calls in this file. 

% If you want to break the section into multiple subsection files, embed
% the \input{subsectionX} calls into the file section.tex

% Subsection files must then stay in the same folder as section.tex,
% and their figures should all stay in the figs/ subdirectory

% All references should included using the bibtex format, and must be
% added to the master report.bib file sitting in the main directory

% If you want to add new tex macros (mostly definitions or new
% commands), include them in your local section.tex file. But first
% make sure you are not overriding the macros already included in the
% main_macros.tex file sitting in the home directory. When processing
% the whole report, each subsection will then call properly its own
% macros, and properly use the master macros

% If you want to collect your macros in a file, you should then input
% it from the file section.tex or 
% from the subsection files, but it should NOT be called
% ``main_macros.tex'' (e.g. call it sectionname_macros.tex)

\input{../header}
\input{../title}
\input{../main_macros}

\input{section}

\bibliographystyle{../report}
\bibliography{smallxhadro}

\end{document}




==> 06-otherhep/report.tex <==
% Few simple rules to ensure that we you can pdfplatex your section
% locally, while maintaining the ability to pdflatex the full
% document from the home directory:

% Don't touch any of the calls in this file. 

% If you want to break the section into multiple subsection files, embed
% the \input{subsectionX} calls into the file section.tex

% Subsection files must then stay in the same folder as section.tex,
% and their figures should all stay in the figs/ subdirectory

% All references should included using the bibtex format, and must be
% added to the master report.bib file sitting in the main directory

% If you want to add new tex macros (mostly definitions or new
% commands), include them in your local section.tex file. But first
% make sure you are not overriding the macros already included in the
% main_macros.tex file sitting in the home directory. When processing
% the whole report, each subsection will then call properly its own
% macros, and properly use the master macros

% If you want to collect your macros in a file, you should then input
% it from the file section.tex or 
% from the subsection files, but it should NOT be called
% ``main_macros.tex'' (e.g. call it sectionname_macros.tex)

\input{../header}
\input{../title}
\input{../main_macros}

\input{section}

\bibliographystyle{../report}
\bibliography{../report}

\end{document}



